Modulation of homogeneous and isotropic turbulence in emulsions

We present a numerical study of emulsions in homogeneous and isotropic turbulence at $Re_\lambda=137$. The problem is addressed via Direct Numerical Simulations (DNS), where the Volume of Fluid (VOF) is used to represent the complex features of the liquid-liquid interface. We consider a mixture of two iso-density fluids, where fluid properties are varied with the goal of understanding their role in turbulence modulation, in particular the volume fraction ($0.03<\alpha<0.5$), viscosity ratio ($0.01<\mu_d/\mu_c<100$) and large scale Weber number ($10.6<We_\mathcal{L}<106.5$). The analysis, performed by studying integral quantities and spectral scale-by-scale analysis, reveals that energy is consistently transported from large to small scales by the interface, and no inverse cascade is observed. Furthermore, the total surface is found to be directly proportional to the amount of energy transported, while viscosity and surface tension alter the dynamic that regulates energy transport. We also observe the $-10/3$ and $-3/2$ scaling on droplet size distributions, suggesting that the dimensional arguments which led to their derivation are verified in HIT conditions.

==> discussion.tex <==


%\subsection{Interpretation of $Re_\lambda$}


\subsection{Spectra and SBS energy balance.}
Overall, analysis in spectral domain reveals some common trends. In all simulations with a dispersed phase, we notice that energy spectra decrease energy at large scales and increase in at small scales. This behavior has already been observed in several works \citep{Perlekar2014,Mukherjee2019,ten2004fully,Rosti2020,Dodd2016,Rosti2020,Olivieri2020a} and it is here confirmed. Interestingly, this behavior seems to be recurrent in most fluids where a dispersed phase, whether solid or liquid, is present in HIT conditions. 

For all cases, we observe that the mechanism of energy transport in SBS energy balance is the same: energy shell-by-shell transfer by the non-linear term decrease, as the surface tension forces absorb energy at large scales. At higher wavenumbers, energy is now transferred through surface tension transport $\mathcal{S}_\sigma$ well within the single-phase dissipative range, forcing dissipation $\mathcal{D}$ to extend its activity into small scales. We report that no inverse cascade has been observed.

With respect to single phase, $\alpha$ is found to be the parameter that most modifies the flow behavior, while it does dot change the underlying physics of the process. This is confirmed in \Cref{sec:res:alpha,sec:res:visc}. Energy transfer via surface tension forces is enhanced at low viscosity ratios, while high viscosity in the carrier phase inhibits the propagation of vortices through the interface, hence dumping energy transport overall. Altering the Weber number result in modulating the crossover frequency at which energy transfer through surface tension directs towards smaller scales. In general, it is shown that, as the dispersed phase becomes more rigid, the energy absorption from the dispersed phase occurs progressively towards larger scales, and turbulence appears to be progressively dumped. In fact, as cohesion forces (either through viscosity or surface tension) increases, more energy is required to deform the dispersed phase, which can only be found in eddies at large scales. 

\MC{The general idea, according to which coalescence and breakup are responsible for generation of spectral deviation with respect to the single phase, seems to explain only partially the behaviors. In fact, according to this theory, largest spectral deviations should be observed while comparing different volume fractions, while viscosity ratio is actually the most influential parameter on spectral deviation. This should be addressed in future studies where coalescence can be inhibit, reduced or controlled numerically.}

\subsection{The role of the Hinze scale.}
%\begin{figure}
%	\centering
%	\includegraphics[width=\textwidth]{figures/ssigma_dsd.eps}
%	\label{fig:ssigma_dsd}
%	\caption{Representation of $\mathcal{S}_\sigma(\kappa)$ on top panel and $PDF(d)$ (represented against $\kappa=2\pi/d$) on bottom panel. $x$-axis are aligned to allow comparison. Black dash-dotted line shows the wavelength where $\mathcal{S}_\sigma$ crosses the $x$-axis; dashed lines represent the $d^{-10/3}$ law from \cite{Garrett2000} (in blue), $d^{-3/2}$ law from \cite{Deane2002} (in red) and Hinze-scale corresponding wavelength in black}
%\end{figure}

Pivoting point is found to be well described by the Hinze scale, also confirming previous results \citep{Perlekar2014, Mukherjee2019}.
% On a novel note, we observe that Hinze scale is also good predictor of the wavelength at which maximum energy is transferred through surface tension forces $\mathcal{S}_\sigma$ from large towards small scales. Although the physical interpretation of this observation is not clearly provided by the data reported, we provide a possible scenario which could justify it. 

%\MC{In a first place, we recall that the term $\mathcal{S}_\sigma$ is the energy transferred through surface tension  at scale $\kappa$, i.e. from shell $\kappa-1$ to shell $\kappa+1$, hence positive when small scales receive energy from large scales. As this term is non-zero only at the interface, it is clearly very intermittent and only droplets with extended interfaces (i.e. large equivalent diameters) will be able to develop large-scale components of this term. As a result, when two droplets coalesce, energy has a path to propagate from small to large scales, hence a negative transfer function can be observed in all cases for $\mathcal{S}_\sigma$. On the contrary, when droplets breaks, energy goes from large towards small scales, as long-wave perturbations on the droplet surface break into disturbances with shorter wavelengths. Droplets of the size of Hinze scale can be formed both by breakup of larger droplets and by coalescence of smaller ones while all smaller droplets.  }

%\Cref{fig:ssigma_dsd} shows the surface tension energy transfer $\mathcal{S}_\sigma$ (top panel) and the DSD ($PDF(d)$, bottom panel) as functions of the wavelength $\kappa$, where the DSD has been represented against $\kappa=2\pi/d$. Dash-dotted black line  shows the wavelength $\kappa_0$ where energy transfer due to surface tension goes to 0. We notice that $\kappa_0$ captures accurately the transition point between the $d^{-3/2}$ and $d^{-10/3}$ power laws, which is usually associated to the Hinze scale in several works \cite{Hinze1975,Deane2002,Mukherjee2019,Perlekar2014}. This does not discredit the reliability of the Hinze scale, rather suggests that the coefficient $0.725$ derived in \cite{Hinze1975} may be inaccurate for the present case, as a significant variability has been observed \cite{Deike:2016ir.Deane2002}. So, what is the meaning of $\kappa_0\approx \kappa_H$ (as $\kappa_0\approx 1.5 \kappa_H$)? We can, in a first place, recall that for $\kappa<\kappa_0$, surface tension absorbs energy from wavelength $\kappa$ ($\mathcal{S}_\sigma<0$), while for $\kappa>\kappa_0$ energy is injected at wavelength $\kappa$. For $\kappa<\kappa_0$, most droplets breaks into smaller ones and coalescence is less likely at relatively high $We$. Through breakup, surface tension energy per unit mass increases, hence energy is absorbed from the carrier flow at that wavelength in order to deform and break the liquid structure. For $\kappa>\kappa_0$ we are in the coalescence regime as droplets cannot further break and only coalescence is possible, which is associated with energy generation as interfacial energy per unit mass is reduced and energy is released into the carrier fluid. 

%In conclusion, Hinze scale is considered as the region where transition occurs between breakup-dominated and coalescence-dominated scales, and the coefficient associated with its definition is indeed subject to significant variations in literature. We show that SBS analysis provide insight beyond turbulence modulation for multiphase flows, as it can also be used to identify with greater accuracy the Hinze scale, as shown in \Cref{fig:ssigma_dsd}. Furthermore, the simultaneous analysis of $\mathcal{S}_\sigma$ and $PDF(d)$ shows a potentially intuitive interpretation for the $-3/2$ and the $-10/3$ power-laws.
   

\subsection{How can we interpret the dissipative range?}
The classical behavior of "deep" dissipation range ($\kappa\sim\kappa_{max}$), where both non-linear energy transport and energy dissipation term in the SBS budget are constantly zero,  is lost when a dispersed phase is introduced. More precisely, non-linear energy transfer still respects this behavior, while energy dissipation does not. As previously stated, data shown suggest that this phenomena is caused by surface tension transfer, which absorbs energy from the non-linear term at large scales and redistributes it at small scales. As previously discussed, energy dissipation reacts by extending towards smaller scales, hence overall increasing the range of wavelength where energy interactions are observed.  In our opinion, increased activity at small scale translates also into an extension ofthe dissipative range, where non-linear transport is substituted by surface tension transport. 

A even more relevant question is "\textit{does that really matter for understanding turbulence in the inertial range?}" In our opinion, an answer to this question is provided in \Cref{subsec:met:sp-case}, where we show and discuss that increasing mesh resolution does not result into any alteration of the inertial range. Therefore, as for a complete discussion on SBS budget resolving the dissipative range is very important, discussions on the inertial range are likely possible even through simulation where surface tension transport is under-resolved.

\subsection{Effects on intermittency.}
We observed through PDFs, mainly of energy dissipation and vorticity, that the presence of a dispersed phase increases intermittency, as probability of distributions tail increases. At higher volume fraction, while viscosity and surface tension are maintained constant, the exponent is independent of the volume fraction. However, the onset of the exponential tail (hence probability of rare event) is affected by $\alpha$, proving that these events are mostly occurring at the interface. modifications of viscosity ratio and surface tension are altered show that intermittency is significantly affected by the fluid properties. In some cases (i.e. low $\mu_d$ and low surface tension), intermittent behavior of vorticity seems to be attenuated worn to single-phase cases. On the other hand, dissipation seems to be constantly affected by the multiphase nature of the flow. 
\MC{Forse serve qualche nota di introduzione ai future studies che abbiamo in mente?}



==> figures/res_alpha.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/r_alpha6c.png}
    \put(-100,140){{$\alpha=0.06$}}
    \includegraphics[width=0.3\textwidth]{figures/r_alpha20c.png}
    \put(-100,140){{$\alpha=0.2$}}
    \includegraphics[width=0.3\textwidth]{figures/r_alpha50c.png}
    \put(-100,140){{$\alpha=0.5$}}
    \caption{ Render of the two-fluid interface (corresponding to the value of the VOF function $\phi=0.5$) for different values of the volume fractions $\alpha$ (left to right, 0.06, 0.2 and 0.5).  The vorticity fields are shown on the box faces on a planar view. }
    \label{fig:alphaRender}
\end{figure}


We first examine  the influence of the dispersed-phase volume fraction on the turbulent flow, cases BE1 and Cxx in \Cref{tab:testMat}, corresponding to increasing values of $\alpha$ from 3 to 50\%. A render of the cases discussed here is shown in \Cref{fig:alphaRender}, where the isocontour of VOF fields are shown for volume fractions $0.06$, $0.2$ and $0.5$. 

The modulation of the turbulence is first quantified in terms of integral quantities.
\Cref{fig:relam_alpha} shows  $Re_\lambda$, computed according to \Cref{eq:relam}, versus the volume fraction $\alpha$. 
$Re_\lambda$ increases  almost linearly with $\alpha$, by approximately 15\% for $\alpha=0.5$.  
A similar trend is found for $\lambda$, as shown in the inset of \Cref{fig:relam_alpha}. Considering that the average of $\varepsilon$ and $k$ is approximately 
constant in all cases (variations of $\pm 3\%$), the increase of $Re_\lambda$ and $\lambda$ is therefore due to  the local variations of the ratio $k/\varepsilon$. 


In particular, the increased values $(k/\epsilon)$ for similar averaged values of the two quantities is attributed to the increased correlation between regions of strong turbulent kinetic energy and low dissipation.
A graphical evidence is presented in \Cref{fig:planes_alpha}, where we show the instantaneous ratio $k/\epsilon$ for the single-phase (case SP2 in panel \textit{a}) and multiphase flow (case BE2 with $\alpha=0.1$ in panel \textit{b}) in logarithmic scale. The figure shows that when the dispersed phase is present,  large regions of fluid with higher $k/\epsilon$ are observed far from the droplet interface (denoted with white line).
This can be explained as follows: as the total dissipation is constant, the local increase of   $\epsilon$ near the interface, as also observed in \cite{Dodd2016}, correspond to a decrease of the dissipation rate in large portions of the fluid, those far from an interface.
Considering that the turbulent kinetic energy is less affected by the presence of the interface, the ratio $(k/\epsilon)$ increases in average.
To support this statement, \Cref{fig:planes_alpha}(\textit{c},\textit{d}) depicts the instantaneous energy dissipation rate for the same planes. In the emulsion
(panel \textit{d}), higher values of $\varepsilon$ are found close to the droplet interface and to the clustering regions, while for the single-phase flow (panel \textit{c}) no specific pattern is observed.


\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{figures/ReLamOnly_alpha.eps}
	\put(-180,65){\includegraphics[width=0.4\textwidth]{figures/LamAlpha_alpha.eps}}
	
	\caption{Taylor Reynolds number, $Re_\lambda$,  versus the dispersed-phase volume fraction $\alpha$, for viscosity ratio $\mu=1$ and density raio $\rho=1$.
	The inset shows the Taylor scale, $\lambda$ versus the different values of $\alpha$ under investigation.}
	\label{fig:relam_alpha}
\end{figure}



\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{figures/k_e_alpha.png}
	\put(-300,130){Single phase}
	\put(-150,130){$\alpha=0.1$}
	\put(-350,120){(\textit{a})}
	\put(-205,120){(\textit{b})}
	
	\includegraphics[width=0.9\textwidth]{figures/eps_plane_alpha.png}
	\put(-350,120){(\textit{c})}
	\put(-205,120){(\textit{d})}
	\caption{(\textit{a,b}) Contours of the ratio $k/\varepsilon$ with logarithmic scale in two planes. (\textit{c,d}) energy dissipation rate $\varepsilon$. The left panels present results for the single phase case SP2, while the right panels results for case BE2 ($\alpha=0.1$). The white lines represent the VOF iso-contours for $\phi=0.5$.}  
	\label{fig:planes_alpha}
\end{figure}



The one-dimensional  energy spectra $E(\kappa)$ multiplied by $\kappa^{5/3}$, i.e.\ the so-called compensated spectra, are displayed in \Cref{fig:spectra_alpha} for the different $\alpha$  considered.
The Taylor scale of the single-phase flow is indicated by the dot-dashed line, while the vertical dotted black line is used for the wavenumber $\kappa_H$ corresponding to the Hinze scale, defined as: 
\begin{equation}
    d_H = 0.725\varepsilon^{-2/5}(\rho_c/\sigma)^{-3/5}.
    \label{eq:hinze}
\end{equation}
Note that,  the prefactor $0.725$ in \Cref{eq:hinze} is set accordingly to the original work of \cite{Hinze1955} for emulsions in HIT conditions,  corresponding to $We_c=1.17$.

The data in \Cref{fig:spectra_alpha} reveal that  the presence of the dispersed phase reduces the energy with respect to the single-phase case (SP1)  for $\kappa<\kappa_H$. At the same time, the energy content increases at the smaller scales, $\kappa>\kappa_H$, in the dissipative range of the spectra. 
As noted in previous studies \citep{Mukherjee2019}, the amount of energy subtracted to the large scales is proportional to the volume fraction $\alpha$. Interestingly, 
the wavenumber at which the curves cross over from reduced to increased energy content corresponds to the Hinze scale. For brevity, we will 
denote as \textit{pivoting point} the wavelength where the spectra of the multiphase cases intersect the one from the single-phase reference case.

Pivoting points were not clearly observed in some previous studies on emulsions \citep{Mukherjee2019, Perlekar2019}, while they are clearly visible in others \citep{Perlekar2014,Dodd2016,Rosti2020};
this is possibly due to the
% A possible explanation for this observation lies in the 
different methods used to simulate the dispersed phase: the ability of the VOF to accurately resolve the interface reduces the energy dissipation by the surface tension term in the dissipative range.  Such energy dissipation is indeed clearly observed by \cite{Perlekar2019} who present results obtained by solving the Cahn-Hilliard equation
in a diffuse-interface formulation. 
As mentioned in \Cref{subsec:met:sp-case}, these numerical artefacts do not have significant effects on the dynamics at the inertial range, while they affect the dissipative range. This aspect will be discussed also later in this section.


\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{figures/spectraComp_alpha.eps}
	\caption{Compensated energy spectra for simulations at different volume fraction $\alpha$; the dot-dashed line represent Taylor scale $\lambda$, while the dotted line the Hinze scale $d_H$.}
	\label{fig:spectra_alpha}
\end{figure}





\begin{figure}
\centering
	\includegraphics[width=0.5\textwidth]{figures/balancefreq_alpha10.eps}
	\put(-200,140){(\textit{a})}
	\includegraphics[width=0.5\textwidth]{figures/fluxTF_alpha.eps}
	\put(-190,140){(\textit{b})}
	
	\includegraphics[width=0.5\textwidth]{figures/surfTF_alpha.eps}
	\put(-200,140){(\textit{c})}
	\includegraphics[width=0.5\textwidth]{figures/dissTF_alpha.eps}
	\put(-190,140){(\textit{d})}
\caption{Scale-by-scale energy budget for different volume fractions $\alpha$. (\textit{a}) Full energy balance for the case BE2 with $\alpha=0.1$; (\textit{b}) the energy transfer $T$ due to the non-linear terms; (\textit{c}) the energy transfer $\mathcal{S}_\sigma$ associated with the surface tension term; (\textit{d}) energy dissipation rate  $\mathcal{D}$.
}
\label{fig:balance_alpha}
\end{figure}



Insight on the energy transfer among the different scales is gained be using the SBS analysis. 
The full SBS energy budegt, i.e.\ the contributions from the different terms in \Cref{eq:spectrBal}, is displayed in 
 \Cref{fig:balance_alpha}(\textit{a}) for case BE2,  chosen as
 an illustrative example with an intermediate value of $\alpha=0.1$. 
The external forcing is injecting energy  at $\kappa=2$, which is absorbed by the non-linear transfer term  $T$, for a large majority, and by the surface tension term $\mathcal{S}_\sigma$, for a small part. The non-linear term transfers energy towards smaller scales, larger values of $\kappa$.
The surface tension term, $\mathcal{S}_\sigma$, acts as a dissipative process at large scales, where it absorbs approximately the same energy as the dissipative term $\mathcal{D}$; however for  $10<\kappa<20$, we observe a significant change in the energy transport mechanism: $\mathcal{S}_\sigma$ becomes positive, hence contributing to transferring energy towards the small scales, similarly to $T$, a process active until $\kappa_{max}$. 
It is important to note that the surface tension transport remains active also at small scales in the dissipative range, consequently extending the range of wavelengths where the dissipation term remains active. These observations confirm the previous findings   obtained in \cite{Perlekar2019} for binary mixtures.

The details of the effect of the volume fraction $\alpha$ on each term of the SBS balance are displayed in \Cref{fig:balance_alpha}(\textit{b-d}). 
We first analyze the non-linear transfer term $T$ in panel (\textit{b}). As $\alpha$ increases, $T$ absorbs progressively less energy at the injection frequency $\kappa=2$. Consequently, less energy is transferred towards smaller scales by nonlinear advection. The energy flux $\Pi$ (not shown) do not display an inverse cascade for any $\alpha$. 
Furthermore, we notice that no energy  is transferred to the far end of the dissipative range, which is resolved over a large range of scales in all cases.    

The contribution from the surface tension $\mathcal{S}_\sigma$, see  \Cref{fig:balance_alpha}(\textit{c}), confirms that interfacial stresses  absorb part of the energy injected into the domain at $\kappa=2$. The energy absorbed by the surface tension term at large scales is approximately proportional to $\alpha$. The surface tension term becomes positive at smaller scales, where energy is released. The positive peak is reached at approximately the Hinze scale for all cases. As for the energy absorption, the magnitude of the peak scales proportionally to $\alpha$. We also notice that, for any $\alpha$, the surface tension terms act also in the dissipative range, where the non-linear term $T$ is zero. 

The behavior observed so far for $T$ and $\mathcal{S}_\sigma$ provide a clear explanation for the previous observations on the energy spectra. At small wavenumber, the energy cascade produced by the non-linear energy transfer is partially inhibited by the presence of the interfacial forces. For high wavenumbers, $T$ progressively reaches zero, but the energy previously subtracted by the interfacial stresses at large scale is redistributed at small scales, which can be seen in \Cref{fig:spectra_alpha} as an energy increase at high wavenumbers.
     

To close the SBS balance, we examine the viscous dissipation term $\mathcal{D}$, see figure \Cref{fig:balance_alpha}(\textit{d}). 
First, we note that only a small amount of the injected energy  (less than $5\%$ for all cases) is absorbed by the dissipation term at the scale of the forcing, $\kappa= 2$.  The overall effect of the dispersed phase is to shift the energy dissipation towards smaller scales. This constitutes the natural reaction of the system to the increased activity in the dissipative range caused by the surface tension term. This behavior becomes more evident as $\alpha$ increases and progressively enhances dissipation at those small scales where the single-phase dissipation  is negligible.

Summarising, the surface tension introduces an alternative path for energy transmission from large towards small scales, as discussed  for binary flows in \cite{Perlekar2019}.
The amount of energy transferred by the surface tension is directly proportional to the total droplets surface area $\mathcal{A}$, as shown in \Cref{fig:dsd_alpha}(\textit{a}) where we display the maximum energy transferred via surface tension $max\left(\sum_{i=1}^{\kappa_{max}}\mathcal{S}_\sigma(i)\right)$ and the total area of the dispersed phase $\mathcal{A}$ for the 
different volume fractions under consideration with a linear fit to the data. This observation 
%suggests 
reinforces our previous conclusion that
 the interface transfers energy among different scales by disrupting larger turbulent structures and creating smaller ones, hence affecting the canonical -5/3 slope of the turbulence spectra.
Note also that, while in mono-dispersed flows this results in a deviation at a specific spectral frequency  \citep{Dodd2016}, in poly-dispersed flows this behaviour is seen at all scales. 


We next consider the dynamics of the dispersed phase.
We first examine  the DSD for all the values of volume fraction studied, see \Cref{fig:dsd_alpha}(\textit{b}),  where we display the droplet diameters normalized by the single-phase (SP1) Kolmogorov scale $\eta_{sp}$

. The dashed black line depicts the $d^{-3/2}$ law by \cite{Deane2002} and the solid line the $d^{-10/3}$ law by \cite{Garrett2000} valid for larger droplets. 
For small droplets, the -3/2 law is well captured also for marginally resolved droplets (with $d/\eta_{sp}<6$). For droplets larger than the Hinze scale, the -10/3 law is also a very good fit, with increasing accuracy for increasing values of $\alpha$. Our data are in agreement with the findings by \cite{Mukherjee2019} and explained by
higher coalescence probability 
 at higher volume fractions,
leading to a bigger population of larger droplets.
Interestingly, the Hinze scale turns out to approximately define the transition between the -3/2 and the -10/3 scalings as proposed in  \cite{Deane2002}, although for higher values of $\alpha$, the onset of the $d^{-10/3}$ power-law occurs at larger diameters.  As the droplet distributions can be, to a good approximation, represented by these 2 laws, it follows that $\mathcal{A}\propto\alpha$, explaining why $\mathcal{A}$, $\mathcal{S}_\sigma$ and $\alpha$ are  linearly correlated (see panel \textit{a} of the same figure).


	

\begin{figure}
\centering
	\centering
	\includegraphics[width=0.49\textwidth]{figures/Area_S_alpha.eps}
	\put(-185,140){(\textit{a})}
	\includegraphics[width=0.49\textwidth]{figures/dsd_alpha.eps}
    \put(-190,140){(\textit{b})}
    
    \includegraphics[width=0.95\textwidth]{figures/legendnosp_alpha.eps}
\caption{(\textit{a}) Correlation between the maximum surface tension term $max\left(\sum_{i=1}^{\kappa_{max}}\mathcal{S}_\sigma(i)\right)$ and the total surface area $\mathcal{A}$ for the different volume fractions $\alpha$. The dashed black line is the linear fit to the data.  (\textit{b}) PDF of the droplet size distribution for different values of $\alpha$. The dashed black line indicates the $d^{-3/2}$ law from \cite{Deane2002}; continuous black line the $d^{-10/3}$ law from \cite{Garrett2000}; dotted black line the Hinze scale $d_H$. The droplet size is normalized by the Kolmogorov scale of simulation SP2 
%	\lb{SP1 or SP2 come sotto??}
	, 
$\eta_{sp}$ .}
\label{fig:dsd_alpha}
\end{figure}



\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{figures/bal_alpha_epsProd.pdf}
	\put(-180,130){(\textit{a})}
	\includegraphics[width=0.5\textwidth]{figures/bal_alpha_tnuTp.pdf}
	\put(-180,130){(\textit{b})}
	\caption{Phase-averaged energy balance versus the dispersed phase volume fraction $\alpha$, see  \Cref{eq:enBalMP}. In each plot, colored triangles (\mytriangle{black}) represent the dispersed phase ($m=d$) while circles (\mycircle{black}) the carrier phase ($m=c$). Each term is normalized by the single phase energy dissipation $\varepsilon_{sp}$ computed for case SP2. The energy production $\mathcal{P}_m$ and energy dissipation $\varepsilon_m$  are reported in panel (\textit{a}), while viscous energy transport $\mathcal{T}^\nu_m$  and the pressure energy transport $\mathcal{T}^p_m$ in panel (\textit{b}).
	}
	\label{fig:balPhase_alpha}
\end{figure}



We now consider the phase-averaged energy budget, introduced in  \Cref{subsec:met:sp-case}. The different terms of \Cref{eq:enBalMP}, production, dissipation and transport by pressure and viscous forces, are shown in \Cref{fig:balPhase_alpha}, normalized by the single-phase dissipation.
We first observe that the total production and dissipation 
\[ \mathcal{P}= \alpha \mathcal{P}_d + (1- \alpha) \mathcal{P}_c \approx\varepsilon\approx 0.95\varepsilon_{sp} \] 
for $\alpha<0.5$.  
The energy production density $\mathcal{P}_m$ (green markers in panel \textit{a}), is higher in the dispersed phase for low volume fractions, while it is comparable to that of the carrier phase for $\alpha>0.1$. 
The energy dissipation rate per unit volume in the dispersed  phase $\varepsilon_d$  (green markers in panel \textit{b}) is also larger at low volume fractions and monotonically decreases with increasing  $\alpha$. 
The dissipation in the carrier phase, $\varepsilon_c$, also decreases, as it compensates for the energy transport $\mathcal{T}_m$ from the carrier flow towards the dispersed phase. 
The viscous transport (see blue markers in panel \textit{b} of the same figure) is significantly lower than its pressure-induced counterpart, $\mathcal{T}^p_m$, although they exhibit a similar behavior: they first increase until  $\alpha=0.1$ and then decrease to reach zero for a binary  mixture.  Note again, that the total transport term is zero, i.e.\ the sum of  $\mathcal{T}^p$ and $\mathcal{T}^{\nu}$ from both phases.
The case $\alpha=0.5$ deserves a specific mention. In this case, production and dissipation in the two phases are equal, hence the transport term $\mathcal{T}_m=0$. Intuitively,  it is not possible to define unambiguously a carrier and dispersed phase in binary mixtures; while the  energy is locally transported from one phase to the other, the global average is zero for both pressure and viscous transfer. 

\begin{figure}
	\centering
	\includegraphics[width=0.33\textwidth]{figures/pdfU_alpha.eps}
	\put(-120,110){(\textit{a})}
	\includegraphics[width=0.33\textwidth]{figures/pdfvort_alpha.eps}
	\put(-120,110){(\textit{b})}
	\includegraphics[width=0.33\textwidth]{figures/pdfeps_alpha.eps}
	\put(-120,110){(\textit{c})}
	
	\includegraphics[width=0.95\textwidth]{figures/legend_alpha.eps}
	\caption{PDF of velocity fluctuations $u$, vorticity $\omega$ and dissipation $\epsilon$. All quantities are normalized as standard score.}
	\label{fig:PDF_alpha}
\end{figure}

We finally analyze the PDF of velocity fluctuations $u_n=u/\sigma_u$, vorticity fluctuations $\omega_n=(|\omega_i|-\langle |\omega_i| \rangle)/\sigma_\omega$ and energy dissipation $\varepsilon_n=(\varepsilon-\langle \varepsilon \rangle)/\sigma_\varepsilon$, normalized by their standard deviation. In \Cref{fig:PDF_alpha}(\textit{a}), we observe that, while the PDF remains symmetric, the tails of the PDF of the velocity fluctuation strongly deviate from the typical pseudo-Gaussian behavior of single-phase turbulence 
\citep{Sreenivasan1997,Jimenez2000a,Ishihara2009}. 
As concerns the vorticity in panel (\textit{b}), no deviation is observed in the Gaussian core \cite[as defined in][]{Sreenivasan1997}. 
However, the distributions of the multiphase flows strongly depart from the single-phase case in the tails. 
In particular, the exponentially decaying tails have a higher exponent in the case of emulsions, indicating more events with strong vorticity.
Interestingly, while increasing the volume fraction does not influence the value of the exponent, increasing $\alpha$ induces deviations in the distributions already at lower values of $\omega_n$. 
% 
We observe  a similar behavior for  $\varepsilon_n$
in panel (\textit{c}):
 the intermittency of the single-phase flow
is amplified by the presence of the interface. As for the vorticity,  departures from the single-phase distributions are observed at lower values of $\varepsilon$  when increasing the volume fraction $\alpha$. 
As a final general remark, the analysis of the PDFs reveals that strong deviations are induced by the presence of the interface, already at low volume fractions,  
overall increasing the intermittent behavior of the flow. As no collapse is observed for the normalized variables, it can be inferred that the small-scale statistics are affected by the presence of the interface.













